The ALMOND Survey: Molecular cloud properties and gas density tracers across 25 nearby spiral galaxies with ALMA

We use new HCN(1-0) data from the ALMOND (ACA Large-sample Mapping Of Nearby galaxies in Dense gas) survey to trace the kpc-scale molecular gas density structure and CO(2-1) data from PHANGS-ALMA to trace the bulk molecular gas across 25 nearby, star-forming galaxies. At 2.1 kpc scale, we measure the density-sensitive HCN/CO line ratio and the SFR/HCN ratio to trace the star formation efficiency in the denser molecular medium. At 150 pc scale, we measure structural and dynamical properties of the molecular gas via CO(2-1) line emission, which is linked to the lower resolution data using an intensity-weighted averaging method. We find positive correlations (negative) of HCN/CO (SFR/HCN) with the surface density, the velocity dispersion and the internal turbulent pressure of the molecular gas. These observed correlations agree with expected trends from turbulent models of star formation, which consider a single free-fall time gravitational collapse. Our results show that the kpc-scale HCN/CO line ratio is a powerful tool to trace the 150 pc scale average density distribution of the molecular clouds. Lastly, we find systematic variations of the SFR/HCN ratio with cloud-scale molecular gas properties, which are incompatible with a universal star formation efficiency. Overall, these findings show that mean molecular gas density, molecular cloud properties and star formation are closely linked in a coherent way, and observations of density-sensitive molecular gas tracers are a useful tool to analyse these variations, linking molecular gas physics to stellar output across galaxy discs.

==> TABLES/Ch_to_ch_corr.tex <==
{\setlength{\tabcolsep}{13pt}
\begin{table}
\resizebox{\columnwidth}{!}{
\begin{threeparttable}[t]
\centering
\caption{Channel-to-Channel Correlation}
\label{TAB:channel_correlation}
\begin{tabular}{ccccc}
\toprule
Galaxy & $r_\mathrm{\ang{;;1}-\ang{;;2}}$ & $r_\mathrm{\SI{75}{\parsec}}$ & $r_\mathrm{\SI{120}{\parsec}}$ & $r_\mathrm{\SI{150}{\parsec}}$ \\\midrule
NGC 0628 & 0.09 & 0.09 & 0.10 & 0.10 \\ 
NGC 1097 & 0.09 & ... & 0.09 & 0.10 \\ 
NGC 1365 & 0.20 & ... & ... & 0.21 \\ 
NGC 1385 & 0.07 & ... & ... & 0.07 \\ 
NGC 1511 & 0.07 & ... & 0.07 & 0.08 \\ 
NGC 1546 & 0.07 & ... & ... & 0.08 \\ 
NGC 1566 & 0.07 & ... & ... & 0.08 \\ 
NGC 1672 & 0.11 & ... & ... & 0.11 \\ 
NGC 1792 & 0.08 & ... & ... & 0.08 \\ 
NGC 2566 & 0.08 & ... & ... & 0.08 \\ 
NGC 2903 & 0.08 & 0.08 & 0.09 & 0.09 \\ 
NGC 2997 & 0.07 & ... & 0.07 & 0.08 \\ 
NGC 3059 & 0.07 & ... & ... & 0.07 \\ 
NGC 3521 & 0.08 & ... & 0.08 & 0.08 \\ 
NGC 3627 & 0.09 & ... & ... & 0.10 \\ 
NGC 4254 & 0.08 & ... & ... & 0.08 \\ 
NGC 4321 & 0.08 & ... & 0.08 & 0.09 \\ 
NGC 4535 & 0.07 & ... & ... & 0.07 \\ 
NGC 4536 & 0.07 & ... & ... & 0.07 \\ 
NGC 5643 & 0.07 & ... & 0.07 & 0.08 \\ 
NGC 6300 & 0.07 & 0.08 & 0.08 & 0.08 \\ 
NGC 7496 & 0.08 & ... & ... & 0.08 \\ 
\bottomrule
\end{tabular}
\begin{tablenotes}
\small
\item 
\end{tablenotes}
\end{threeparttable}
}
\end{table}
}

==> title.tex <==
% Name + Affiliation + Acknowledgements

% Please append below! 

% Miguel Querejeta, Observatorio Astron{\'o}mico Nacional (IGN), C/ Alfonso XII 3, E-28014 Madrid, Spain ---- MQ acknowledges support from the Spanish grant PID2019-106027GA-C44, funded by MCIN/AEI/10.13039/501100011033.

% Jiayi Sun
% \thanks{CITA National Fellow}
% Department of Physics and Astronomy, McMaster University, 1280 Main Street West, Hamilton, ON L8S 4M1, Canada
% Canadian Institute for Theoretical Astrophysics (CITA), University of Toronto, 60 St George Street, Toronto, ON M5S 3H8, Canada
% \OSU
% The work of JS is partially supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) through the Canadian Institute for Theoretical Astrophysics (CITA) National Fellowship.

% Yu-Hsuan Teng
% Center for Astrophysics and Space Sciences, Department of Physics, University of California San Diego, 9500 Gilman Drive, La Jolla, CA 92093, USA
% Y.-H.T. acknowledges funding support from NRAO Student Observing Support Grant SOSPADA-012 and from the National Science Foundation (NSF) under grant No. 2108081.

% Daizhong Liu
% [0000-0001-9773-7479]
% Max-Planck-Institut f\"ur Extraterrestrische Physik (MPE), Giessenbachstr. 1, D-85748 Garching, Germany

% Mattia C. Sormani
% ORCID: 0000-0001-6113-6241
% AFFILIATION: Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Institut f\"{u}r theoretische Astrophysik, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany \\
% ACKNOWLEDGEMENTS: MCS acknowledges financial support from the European Research Council via the ERC Synergy Grant ``ECOGAL - Understanding our Galactic ecosystem: from the disk of the Milky Way to the formation sites of stars and planets'' (grant 855130).

% Ralf S.\ Klessen
% ORCID: 0000-0002-0560-3172
% Affiliation 1:  Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Institut f\"{u}r theoretische Astrophysik, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany 
% Affiliation 2: Universit\"{a}t Heidelberg, Interdisziplin\"{a}res Zentrum f\"{u}r Wissenschaftliches Rechnen, Im Neuenheimer Feld 205, \\ D-69120 Heidelberg, Germany  
% Acknowledgements (can be combined with Glover/Sormani): R.S.K. acknowledges financial support from the Heidelberg cluster of excellence (EXC 2181 - 390900948) “{\em STRUCTURES}: A unifying approach to emergent phenomena in the physical world, mathematics, and complex data”. R.S.K. also thanks for support from Deutsche Forschungsgemeinschaft (DFG) via the Collaborative Research Center (SFB 881, Project-ID 138713538) 'The Milky Way System' (subprojects A01, A06, B01, B02, and B08). And he thanks for funding form the European Research Council in the ERC synergy grant “{\em ECOGAL} – Understanding our Galactic ecosystem: From the disk of the Milky Way to the formation sites of stars and planets” (project ID 855130). 

% Yixian Cao
% [0000-0001-5301-1326]
% Max-Planck-Institut f\"ur Extraterrestrische Physik (MPE), Giessenbachstr. 1, D-85748 Garching, Germany

% Mar\'ia J. Jim\'enez-Donaire
% Observatorio Astron\'omico Nacional (IGN), C/Alfonso XII, 3, E-28014 Madrid, Spain
% and
% Centro de Desarrollos Tecnol\'ogicos, Observatorio de Yebes (IGN), 19141 Yebes, Guadalajara, Spain

%Kathryn Grasha
% orcid; 0000-0002-3247-5321
%Affiliation: 
%Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia
% and
% ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia

% M\'{e}lanie~Chevance\orcidlink{0000-0002-5635-5180}
% Affiliation: Astronomisches Rechen-Institut, Zentrum f{\"u}r Astronomie der Universit{\"a}t Heidelberg, M{\"o}nchhofstra{\ss}e 12-14, 69120 Heidelberg, Germany
% Acknowledgements (can be combined with Kruijssen): MC gratefully acknowledges funding from the Deutsche Forschungsgemeinschaft (DFG) through an Emmy Noether Research Group (grant number KR4801/1-1) and the DFG Sachbeihilfe (grant number KR4801/2-1), as well as from the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation programme via the ERC Starting Grant MUSTANG (grant agreement number 714907).

% J.~M.~Diederik Kruijssen\orcidlink{0000-0002-8804-0212}
% Affiliation: Astronomisches Rechen-Institut, Zentrum f{\"u}r Astronomie der Universit{\"a}t Heidelberg, M{\"o}nchhofstra{\ss}e 12-14, 69120 Heidelberg, Germany
% Acknowledgements (can be combined with Chevance): JMDK gratefully acknowledges funding from the Deutsche Forschungsgemeinschaft (DFG) through an Emmy Noether Research Group (grant number KR4801/1-1) and the DFG Sachbeihilfe (grant number KR4801/2-1), as well as from the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation programme via the ERC Starting Grant MUSTANG (grant agreement number 714907).
